Graph Sampling for Matrix Completion Using Recurrent Gershgorin Disc Shift

Matrix completion algorithms fill missing entries in a large matrix given a subset of observed samples. However, how to best pre-select informative matrix entries given a sampling budget is largely unaddressed. In this paper, we propose a fast sample selection strategy for matrix completion from a graph signal processing perspective. Specifically, we first regularize the matrix reconstruction objective using a dual graph signal smoothness prior, resulting in a system of linear equations for solution. We then select appropriate samples to maximize the smallest eigenvalue $\lambda_{\min}$ of the coefficient matrix, thus maximizing the stability of the linear system. To efficiently solve this combinatorial problem, we derive a greedy sampling strategy, leveraging on Gershgorin circle theorem, that iteratively selects one sample (equivalent to shifting one Gershgorin disc) at a time corresponding to the largest magnitude entry in the first eigenvector of a modified graph Laplacian matrix. Our algorithm benefits computationally from warm start as the first eigenvectors of incremented Laplacian matrices are computed recurrently for more samples. To achieve computation scalability when sampling large matrices, we further rewrite the coefficient matrix as a sum of two separate components, each of which exhibits block-diagonal structure that we exploit for alternating block-wise sampling. Extensive experiments on both synthetic and real-world datasets show that our graph sampling algorithm substantially outperforms existing sampling schemes for matrix completion and reduces the completion error, when combined with a range of modern matrix completion algorithms.

==> bandlimitedSampling.tex <==
Besides proposing a new generic graph sampling method (GCS) and its iterative variant IGCS for active matrix completion, we will formulate another sampling framework in this section based on \emph{dual bandlimited assumption}, which is extended from sampling on single graphs \cite{wang18}. 
%This formulation is mainly derived from the assumption that the matrix signal is \emph{bandlimited} on dual graphs. 

\subsection{Support Graph}
From section \ref{sec:formulate}, we know that the original matrix signal $\X$ is dual-smooth with respect to row graph $\L_r$ and column graph $\L_c$.  
Once we rewrite the matrix information $\X$ into a vector information, we should find its corresponding supported one-dimensional graph with size $mn$. 
We first prove the following lemma:
\begin{lemma}
If $\emph{\text{Tr}}\left(\mathbf{X}^{T}\mathbf{L}_{r}\mathbf{X}\right)<\gamma_1$ and $\emph{\text{Tr}}\left(\mathbf{X}\mathbf{L}_{c}\mathbf{X}^{T}\right)<\gamma_2$, then 
\begin{equation}
    \x^T(\mathbf{I}_n\otimes\mathbf{L}_{r}
+\mathbf{L}_{c}\otimes\mathbf{I}_m)\x<\gamma_1+\gamma_2
\end{equation}
where $\x=\text{vec}(\X)$
\end{lemma}
\begin{proof}
Since $\text{Tr}(\A^T\B)=\text{vec}(\A)^T\text{vec}(\B)$, $\text{Tr}\left(\X^{T}\mathbf{L}_{r}\mathbf{X}\right)=\text{vec}(\X)^T\text{vec}(\L_r\X)$ and $\text{Tr}\left(\mathbf{X}\mathbf{L}_{c}\mathbf{X}^{T}\right)=\text{Tr}\left(\mathbf{X}^{T}\mathbf{X}\mathbf{L}_{c}\right)=\text{vec}(\X)^T\text{vec}(\X\L_c)$. 
Recall the property used in section \ref{sec:formulate} that 
$\text{vec}(\L_r\X)=(\I_n\otimes\L_r)\text{vec}(\X)$ and $\text{vec}(\X\L_c)=(\L_c\otimes\I_m)\text{vec}(\X)$, we have the result that 
$\x^T(\mathbf{I}_n\otimes\mathbf{L}_{r}
+\mathbf{L}_{c}\otimes\mathbf{I}_m)\x=\text{Tr}\left(\mathbf{X}^{T}\mathbf{L}_{r}\mathbf{X}\right)+\text{Tr}\left(\mathbf{X}\mathbf{L}_{c}\mathbf{X}^{T}\right)<\gamma_1+\gamma_2$.
\end{proof}

This lemma means that the vectorial graph signal is smooth with respect to the Cartesian product Laplacian (also known as Kronecker sum ) $\L_p=\mathbf{I}_n\otimes\mathbf{L}_{r}
+\mathbf{L}_{c}\otimes\mathbf{I}_m$ if the original matrix data $\X$ is smooth on double graphs. 
This is a specific product graph introduced in paper \cite{PG}. In this paper, we will use this product graph as the support graph for a matrix signal $\X$. 

\begin{comment}
From the vertex domain, it is observed that 
\begin{align}
&\hspace{-0.5cm}
    \Z(i,j)=(\L_r\X+\X\L_c)(i,j)\nonumber\\
&
    =\d_r(i)\X(i,j)-\sum_{k\in\mathcal{N}_r(i)}\W_r(i,k)\X(k,j)\\
&
    +\d_c(j)\X(i,j)-\sum_{t\in\mathcal{N}_c(j)}\W_c(j,t)\X(i,t)\nonumber
\end{align}
where $\Z$ is the matrix version of vector $\z=\L_p\x$, $\mathcal{N}_r(i)$ and $\mathcal{N}_c(j)$ are the neighbor set of node $i$ in row graph and that of node $j$ in column graph. 
Assume $\bar{\x}$ is the solution of system $\L_p\x=0$, i.e., $\L_r\bar{\X}+\bar{\X}\L_c=\mathbf{0}$, then 
\begin{equation}
    \bar{\X}(i,j)=\frac{\sum_{k\in\mathcal{N}_r(i)}\W_r(i,k)\bar{\X}(k,j)+\sum_{t\in\mathcal{N}_c(j)}\W_c(j,t)\bar{\X}(i,t)}{\d_r(i)+\d_c(j)}
\end{equation}
This can be seen as an extension of \emph{harmonic} solution from one-dimensional graph to dual-graph domain introduced in \cite{zhu2003icml}. 
From this equation, we know that for the harmonic solution, signal energy on each node is the weighted average of all its neighbors' energy in the dual graphs, similar to one-dimension harmonic graph signal on a single graph. 
This indicates that the supported graph $\L_p$ is a reasonable graph for expressing the vectorized signal $\x$.
\end{comment}

%\subsection{Sampling under Bandlimited Assumption}
After classifying the underneath support graph, we now introduce how to use the conventional graph sampling methods on this graph, thus extending graph sampling into active matrix completion.

\subsection{Sampling on Product Graph with Bandlimited Assumption}
Authors in \cite{anis16} proposed a lightweight graph sampling method based on \emph{spectral proxies} (SP), which can collect nodes on $\L_p$ directly and requires the first eigenvector of a submatrix in each greedy step. 
Besides, an eigen-decomposition free method was proposed in \cite{akie2018eigenFREE} to perform sampling on a localized operator on the product graph, which can be implemented by a Chebyshev polynomial of $\L_p$.
%in \cite{chen15sampling,wang18,chamon2018}. 
There are also some other graph sampling methods which exploit the eigenspace information of the Laplacian $\L_p$ to conduct sampling. However, the dimension of $\L_p$ is $mn$, so the complexity of its eigen-decomposition is $m^3n^3$ in general,  which is really a huge cost. 
Luckily, as shown in \cite{kronecker}, the eigenvector matrix of $\L_p$ is $\U \otimes \V$, where $\U\in\mathbb{R}^{n\times n}$ and $\V\in\mathbb{R}^{m\times m}$ are the eigenvector matrix of $\L_c$ and $\L_r$ respectively. Based on this property, the complexity of eigen-decompsition is $\cO(m^3+n^3)$. Since the matrix graph signal is smooth in both row graph and column graph, its spectral expression can be formulated as \cite{PG}
\begin{equation}
    \x=(\U \otimes \V)\tilde{\x} \Longleftrightarrow \X=\V\tilde{\X}\U^T
\end{equation}
where $\tilde{\x}$ is the GFT of signal $\x$, and $\tilde{\X}$ is its matrix form. 

Once the matrix signal is restricted to be bandlimited in both row graph and column graph, it will have a low dimensional expression based on the first $k_1$ eigenvectors of $\L_c$ and first $k_2$ eigenvectors of $\L_r$, where $k1\ll n$ and $k2\ll m$. 
\begin{equation}
    \X=\V_{k_2}\tilde{\X}_f\U^T_{k_1} \Longleftrightarrow \x=(\U_{k_1}\otimes\V_{k_2})\tilde{\x}_f
\end{equation}
where $\tilde{\X}_f$ means the submatrix of $\X$ on its first $k_2$ rows and first $k_1$ columns and $\tilde{\x}_f=\text{vec}(\tilde{\X}_f)$; $\U_{k_1}$ is a tall matrix formed by the first $k_1$ columns of $\U$ and $\V_{k_2}$ is  constructed by the first $k_2$ columns of $\V$. 

To realize $\U_{k_1}\otimes\V_{k_2}$, the whole complexity is $\cO(m^3+n^3+k_1k_2mn)$, which is much lower than $\cO(m^3n^3)$. 
This is a case named as \emph{dense core tensor}-based linear system in \cite{tensor}. 
In paper \cite{huang2018matrix}, a special case where the core tensor is exactly diagonal, is proposed to enhance the matrix completion method, where the graph is constructed via rating information. 

%Authors in \cite{PG} proposed \emph{structured sampling} to select nodes from row and column separately, since they . 
If we want to perform \emph{unstructured sampling} on the matrix data using other published deterministic graph sampling strategies, we can see  $\U_{k_1}\otimes\V_{k_2}$ as the supported eigenvector matrix of $\x$. Based on partial observations $\y_{\cS}=\C(\U_{k_1}\otimes\V_{k_2})\tilde{\x}_f+\n_{\cS}$, Least square (LS) reconstruction is used for recovery if $\textrm{rank}[\C(\U_{k_1}\otimes\V_{k_2})]\ge k_1k_2$ \footnote{$\textrm{rank}(\U_{k_1}\otimes\V_{k_2})=\textrm{rank}(\U_{k_1})\textrm{rank}(\V_{k_2})=k_1k_2$}: 
\begin{equation}
    \begin{split}
&        \hat{\x}=(\U_{k_1}\otimes\V_{k_2})\left[\C(\U_{k_1}\otimes\V_{k_2})\right]^{\dag}\y_{\cS}
    \end{split}
\end{equation}
where $\dag$ denotes the pseudo-inverse computation and $\C$ is the sampling operator on dual graph with sampling set $\cS$ defined in \eqref{sampleset} such that 
\begin{equation}
\begin{split}
{{\mathbf{C}(k,l)} = \left\{ \begin{array}{l}
1,~~~{l = {\mathcal{S}(k)}};\\
0,~~~\textrm{otherwise},
\end{array} \right.}
\end{split}
\end{equation}

It is easy to verify that 
$\C^T\C=\tilde{\mathbf{A}}_{\Omega}=\text{diag}(\text{vec}({\mathbf{A}}_{\Omega}))$.
Based on A-optimal objective sampling function used in \cite{wang18}, the sampling function on dual graph can be generalized as 
\begin{equation}\label{AoptimalMC}
    \min_{\C}~~h(\C)=\text{Tr}\left[(\U_{k_1}\otimes\V_{k_2})^T\C^T\C(\U_{k_1}\otimes\V_{k_2})\right]^{-1}
\end{equation}


\input{tableBLSM}

E-optimal criterion can be used as a worst case of A-optimal objective via optimizing 
\begin{equation}
    \max_{\C}~~\sigma_{\min}\left[\C(\U_{k_1}\otimes\V_{k_2})\right]
\end{equation}
which can be regarded as an extension of method used in single graph sampling in paper \cite{chen15sampling}.

The above formulated problems are all combinatorial and generally optimized via greedy method in the graph sampling field. While classical graph sampling methods can be used for matrix completion,  authors in \cite{PG,tensor} argued that unstructured sampling doesn't involve any factorizations of the product graph, thus its complexity scales with total  number of vertices ($mn$) and its practicability is limited. 
%They claimed that classical sampling is not applicable to signals supported by large product graphs. 
In this paper, we want to show the following viewpoints about the applicability of those classical sampling methods:
\begin{itemize}
    \item Though the size of product graph is $mn$, classical graph sampling methods never perform eigen-decomposition on $\L_p$ directly, but on $\L_r$ and $\L_c$ separately as discussed. 
    \item Ignoring the influence from sample size and initial eigen-decomposition for $\U$ and $\V$, the complexity of classical sampling methods scale \textbf{linear} to the graph size $mn$ since the size of greedy search pool is $mn$. As we know, in conventional active matrix complexion field, the size of searching pool for active querying is also $mn$ \cite{activeMC2015}. It is not precise to state that classical sampling is not applicable at all to active matrix completion work. 
    \item Some local search strategy can be utilized to reduce the complexity, like random group search proposed in \cite{aggressive2018TSIPN}. In the following content, we will propose one local search strategy based on the GCS method. 
    \item The newly proposed sampling method GCS scales linear to $mn$ but the heuristic one IGCS is linear to $m$ or $n$, which mainly  targets on lower complexity. 
\end{itemize}

\subsection{A-optimal Sampling with GCS-based Local Search Pool}
In this paper, we want to implement the classical A-optimal sampling strategy for matrix completion problem. However, as we discussed, the greedy search pool is of size $mn$, which implies that collecting one new sample requires evaluation on all left $\cO(mn)$ candidates. This complexity is not urgent in single graph sampling, but in dual graph sampling, $mn$ could be too large to perform greedy evaluation even when $m$ and $n$ are not large.  

Recall that the proposed GCS sampling is to sample node whose supported signal's energy is the largest one. If we choose the top $L$ node  with large signal energy for candidates of the A-optimal sampling, the complexity of the classical A-optimal sampling would be reduced tremendously. The detailed algorithm of A-optimal sampling with local search is illustrated in Algorithm \ref{AoL}, where ``descend'' is a function to produce the corresponding index set of descend-ranked vector $\bphi$. $\cA(1:L)$ is a set of the first $L$ elements in set $\cA$. 

\begin{algorithm}[tp]
\caption{A-optimal Sampling with Local Search Pool}
\label{AoL}
\textbf{Input}: Sample budget $K$; $\T=\U_{k_1}\otimes\V_{k_2}$; $\L=\alpha\mathbf{I}_n\otimes\mathbf{L}_{r}+\beta\mathbf{L}_{c}\otimes\mathbf{I}_m$; Local search size $L$.\\
\textbf{Initialization}: $\cS=\{\varnothing\}$
\begin{algorithmic}[1]
\State While $|\cS|<K$
\State compute the first eigenvector $\pmb{\phi}$ of $\L$
\State $\bar{\bphi}=|\bphi|$, $\bar{\bphi}(\cS)=-1$
\State $\cA=\textrm{descend}(\bar{\bphi})$ and $\cB=\cA(1:L)$
\State $i^* \gets \min_{i\in\cB}h(\cS\cup\{i\})$
\State $\cS \gets \cS\cup\{i^*\}$
\State Update $\L=\L+\e_{i^*}\e^T_{i^*}$
\State end While
\State return $\cS$
\end{algorithmic}
\end{algorithm}

Note that in this paper, we not only propose two new sampling methods, named as GCS and IGCS, but also extend classical graph sampling methods into dual graphs, using the A-optimal sampling as an example. Our main argument is that unstructured graph sampling is applicable for matrix completion problem with some local search strategies. 
Authors in \cite{PG} sacrifice the flexibility of arbitrary sample budget for achieving considerable complexity, which is actually not worthwhile. 

\subsection{Smootheness versus Bandlimitedness}
%In this paper, we mainly focus on proposing the GCS and IGCS sampling method based on dual graph smoothness prior. Further, we extend the sampling objective function from classical single graph sampling to dual graph sampling via bandlimitedness assumption. 
In this subsection, we give a comprehensive analysis between proposed sampling strategy (GCS and IGCS) and other sampling strategies: 
\begin{itemize}
    \item Compared with SP sampling on $\L_p$, the GCS method doesn't have  to manipulate on $k$ degree of the Laplacian, but operate sampling on $\L$ (section \ref{sec:sampling1}) directly. The degree $k$ enlarges the number of iterations of LOBPCG for convergence. 
    In each internal greedy iteration, the GCS will use the previous eigenvector as an initial guess of the next eigenvector to accelerate the convergence of the LOBPCG method, which cannot be utilized in SP method. Both of those will make the GCS method more efficient than SP method. 
    \item Compared with A-optimal sampling or E-optimal sampling without local search, the proposed GCS sampling doesn't assume any bandlimitedness property but use the dual-graph smoothness property, which is more practical since dual bandwidth $k_1$ and $k_2$ are unknown. Further, the GCS method doesn't have to compute the first $k_1$ and $k_2$ eigenvectors or evaluate a computational objective value in each greedy step. 
    \item Compared with the PG method \cite{PG}, the proposed IGCS has comparable complexity since it also operates between the factor graphs iteratively by exploiting the block diagonal structure in $\Q$. Further, it is an unstructured sampling for matrix completion problem,  thus more practical and flexible. In contrast, the samples from PG sampling consist of a rectangular sampling submatrix and the sample size of PG method is unpredictable before finishing sampling. 
\end{itemize}

We list some properties of different sampling strategies for matrix completion in Table \ref{analysis}. In Table \ref{analysis}, ``Greedy pool'' the size of candidates of  greedy evaluation for collecting each new sample and ``per Evaluation'' denotes the worst complexity inner each greedy search.  
It is obvious that the proposed GCS sampling doesn't involve $\U$ and $\V$, and doesn't evaluate $mn$ candidates, thus leading to considerable complexity compared with classical graph sampling methods. 
Though IGCS has lower complexity than the proposed GCS method, its performance will deteriorate because it is a heuristic proposal . 
In experiments, we will simulate random sampling, the proposed Algorithms \ref{GCS}, \ref{IGCS} and \ref{AoL} and PG sampling in \cite{PG} on comprehensive sythetic and real-world datasets for performance comparison.  

==> sampling.tex <==
We first discuss our sampling strategy based on Gershgorin disc alignment for a general single graph in Section\;\ref{subsec:sampling1}. 
We then discuss our methodology to apply the single-graph sampling algorithm to the dual graph for matrix completion in Section\;\ref{subsec:sampling2}.

\subsection{Gershgorin-disc-based Sampling}
\label{subsec:sampling1}

Most existing graph sampling works that require computation of extreme eigenvectors to greedily determine the next sample until a pre-determined sampling budget is met.
In contrast, we select samples to maximize the lower bound of the minimum eigenvalue of a graph Laplacian matrix via Gershgorin disc alignment, which requires no explicit computation of any eigenvalues or eigenvectors. 
Thus our sampling algorithm is significantly faster than previous graph sampling proposals; we discuss algorithmic complexity comparison in details later.

\subsection{Preliminaries}
\label{subsec:prelim}

We first overview the well-known \textit{Gershgorin circle theorem} (GCT) \footnote{https://en.wikipedia.org/wiki/Gershgorin\_circle\_theorem} in linear algebra.
Given a square matrix $\A$, the $i$-th \textit{Gershgorin disc}, corresponding to the $i$-th row of $\A$, has center $c_i = \sum_{j} A_{i,j}$ and radius $r_i = \sum_{j \neq i} |A_{i,j}|$.
GCT states that the smallest eigenvalue $\lambda_{\min}$ of $\A$ is lower bounded by the smallest left-ends of all Gershgorin discs, 
\begin{align}
\lambda_{\min} \geq \min_i ~ \left\{ c_i - r_i \right\}
\label{eq:GCT}
\end{align}
where $c_i - r_i$ is the left-end of the $i$-th Gershgorin disc.
Notice that the computation of this smallest eigenvalue lower bound (\ref{eq:GCT}) involves simple addition without any complex eigenvalue computation such as the Lanczos algorithm \red{add ref}.

We state next a linear algebra fact (without proof for brevity) that we exploit for our algorithm:
\begin{quotation}
Matrix $\S \, \A \, \S^{-1}$ with \textit{similarity transform} matrix $\S$ has the same set of eigenvalues as matrix $\A$, assuming $\S$ is invertible.
\end{quotation}
It is known that the GCT lower bound (\ref{eq:GCT}) for $\lambda_{\min}$ is often too loose to be useful directly.
Given the above fact, one strategy is to design similarity transform $\S$ so that the Gershgorin discs of $\A' = \S \, \A \, \S^{-1}$ provide a tighter lower bound for $\lambda_{\min}$.
%We discuss our strategy when $\A$ is a graph Laplacian matrix $\L$ in the context of graph sampling next. 

\subsection{Disc Alignment Problem}
\label{subsec:discAlign}

By definition of a combinatorial graph Laplacian matrix $\L = \D - \A$ for a positive-edge-weighted graph $\cG$, where $L_{i,i} = D_{i,i} = \sum_{j \neq i} A_{i,j}$ and $L_{i,j} = -A_{i,j} \leq 0, \forall i \neq j$, we observe that the left-end of each Gershgorin disc $i$, $c_i - r_i$, is exactly at $0$.
By GCT, it means that the lower bound of $\lambda_{\min}$ for graph Laplacian $\L$ is 0, which is a well-known fact in the GSP literature\;\cite{ortega18ieee,cheung18}. 

Denote by $\D \in \{0, 1\}^{M \times N}$ a \textit{sampling matrix} that extracts $M$ chosen elements from a vector $\x \in \mathbb{R}^{N}$. 
We next define a \textit{sampled graph Laplacian matrix} $\L_s = \D^{\top} \D + \mu \L$ as a weighted sum of sampling matrix $\D$ times its transpose and a graph Laplacian matrix $\L$.
$\D^{\top} \D \in \{0, 1\}^{N \times N}$ is a diagonal matrix with $1$'s at diagonal entries corresponding to the sampled nodes and $0$ elsewhere. 
Thus $\L_s$ can be interpreted as a modified graph Laplacian matrix with additional \textit{self-loops} of weight $1$ at sampled nodes. 
For each $i$-th row of $\L_s$ where $i$ is a sampled node, by GCT it means that the corresponding Gershgorin disc center $c_i$ (and consequently the disc's left-end $c_i - r_i$) is shifted to the right by $1$.

Define now a \textit{scaled Laplacian matrix} $\B = \S  \, \L_s \, \S^{-1}$, where similarity transform $\S \in \mathbb{R}^{N \times N}$ is a diagonal matrix with \textit{scale factors} $s_1, \ldots, s_N$, $s_i > 0, \forall i$, along its diagonal. 
By restricting similarity transform $\S$ to be a diagonal matrix with a trivial matrix inverse $\S^{-1} = \mathrm{diag}(1/s_1, \ldots, 1/s_N)$, one can narrowly focus on selection of diagonal entries $s_1, \ldots, s_N$ that maximizes the smallest left-ends of Gershgorin discs of $\B$, towards the goal of obtaining a tight lower bound for $\lambda_{\min}$ of the original matrix $\L_s$.

Given the above definitions, we can now define the graph sampling problem as follows. Given a budget of $\bar{H}$ samples, select no more than $\bar{H}$ out of $N$ nodes for sampling, so that together with scale factors $s_1, \ldots, s_N$, the $\lambda_{\min}$ lower bound of $\L_s$, as computed as the smallest left-end of all Gershgorin discs in $\B = \S \, \L_s \, \S^{-1}$, is maximized. 
We formulate this optimization mathematically as follows:
\begin{align}
\max_{\{s_i\}, \{e_i\}} &
\min_{i} \left\{ c_i - r_i \right\} 
\label{eq:discAlign} \\
\mbox{s.t.} \; & c_i = B_{i,i}, \;\;\; r_i = - \sum_{j \neq i} B_{i,j} \nonumber \\
& \B = \S \left (\E + \mu \L \right ) \S^{-1}, 
\;\;\; \S = \mathrm{diag}(s_1, \ldots, s_N)
\nonumber \\
& \E = \mathrm{diag}(e_1, \ldots, e_N), 
\;\; \sum_{i=1}^N e_i \leq \bar{H}, 
\;\; e_i \in \{0, 1\}
\nonumber 
\end{align}
where we replace $\D^{\top} \D$ with diagonal matrix $\E$ for simplicity. 
Since $B_{i,j} \leq 0, \forall i \neq j$, disc radius $r_i$ is the negative sum of the non-diagonal entries $B_{i,j}$ on row $i$.

(\ref{eq:discAlign}) is a difficult problem to tackle given the combinatorial nature in $\{e_i\}$ and multiplicative inter-variable dependency in $\{s_i\}$ when $\B$ is computed. 
To solve (\ref{eq:discAlign}) efficiently, we propose a dynamic programming (DP) algorithm discussed next.


\subsection{Dynamic Programming Algorithm}
\label{subsec:DP}

One inherent difficulty of (\ref{eq:discAlign}) is the max-min criterion, which is difficult to optimize in general.
We thus repose the problem as follows:
\begin{align}
\min_{\{s_i\}, \{e_i\}} & \sum_{i=1}^N e_i 
\label{eq:discAlign2} \\
\mbox{s.t.} \;\; & c_i = B_{i,i}, \;\;\; r_i = - \sum_{j \neq i} B_{i,j}, \;\;\;  c_i - r_i \geq \delta_{\min}, \; \forall i \nonumber \\
& \B = \S \left (\E + \mu \L \right ) \S^{-1}, 
\;\;\; \S = \mathrm{diag}(s_1, \ldots, s_N)
\nonumber \\
& \E = \mathrm{diag}(e_1, \ldots, e_N), 
\;\;\; e_i \in \{0, 1\}
\nonumber 
\end{align}
where $\delta_{\min}$ is the \textit{disc threshold} and a parameter for optimization (\ref{eq:discAlign2}).
In words, in (\ref{eq:discAlign2}) we swap the roles of the max-min objective in discs' left-ends $c_i - r_i$ with the constraint on $\sum_{i=1}^N e_i$, so that both the new objective and constraint in (\ref{eq:discAlign2}) become linear.
One can show that if $\delta_{\min}$ is chosen such that there exists an optimal solution $(\{s_i^*\}, \{e_i^*\})$ to (\ref{eq:discAlign2}) satisfying $\sum_{i=1}^N e_i^* = \bar{H}$, then one optimal solution to (\ref{eq:discAlign2}) is also an optimal solution to (\ref{eq:discAlign}). 
(See Appendix\;\ref{subsec:append1} for a short proof.) 
The new difficulty is thus how to search for such $\delta_{\min}$ (if it exists). 
We defer this discussion to Section\;\ref{subsec:singular}, and focus first on solving (\ref{eq:discAlign2}) for a given disc threshold $\delta_{\min}$.

\subsubsection{NP-Hardness of Node Ordering}

\red{discuss the potential NP-hardness of ordering nodes.}

\subsubsection{Definition of DP Algorithm}

We devise a DP algorithm for (\ref{eq:discAlign2}) as follows given node visiting order is fixed. 
We first define an ordered list of $N$ nodes, $\cV = \{v_1, \ldots, v_N\}$, where $v_i \in \{1, \ldots, N\}$ and $v_i \neq v_j$ if $i \neq j$, that specifies the order in which the $N$ nodes are visited. 
We define a \textit{boundary set} $\phi_t$ as the subset of visited nodes $\cV_t = \{v_1, \ldots, v_t\}$ at instant $t$ with connectivity to the remaining unvisited nodes $\bar{\cV}_t = \{v_{t+1} \ldots, v_N\}$. 
$\phi_t$ and $\phi_t{-1}$ are related as follows:
\begin{align}
\phi_t \subseteq \phi_{t-1} \cup \{v_t\}
\label{eq:phi_t}
\end{align}
\eqref{eq:phi_t} means that one can simply check for connectivity of only $\phi_{t-1}$ and $v_t$ with $\bar{\cV}_t$ to determine $\phi_t$. 
$\phi_t$ is the set of nodes whose scale factors we carry forward to the next recursive call. 

We now describe a recursive algorithm \texttt{MINSAMP}$(t, \s_{\phi_t})$ that returns the minimum number of samples at instant $t$ given scale factors $\s_{\phi_t}$ of the boundary set $\phi_t$. 
At each instant $t$, we first update radius $r_{v_t}$ given scale factors $\s_{\phi_t}$:
\begin{align}
r_{v_t} = - \sum_{j \neq v_t}
\frac{L_{i,j}}{s_{j}}
\label{eq:updateRadius}
\end{align}
We then check if the Gershgorin disc left-end $c_{v_i} - r_{v_i}$ of newly visited node $v_i$ is above threshold $\delta_{\min}$.
If so, then there are two possible choices.
First, one can sample node $v_i$ and compute scale factor $s_{v_i}$ as:
\begin{align}
s_{v_i} &= \frac{c_{v_i} - \delta_{\min}}{r_{v_i}}
\label{eq:scale0}
\end{align}
$s_{v_i} \geq 1$ since we know $c_{v_i} - r_{v_i} > \delta_{\min}$.
$s_{\phi_{t+1}}$ can be defined given $s_{\phi_t}$ and $s_{v_i}$. 
The cost for this choice is $c_0 = \texttt{MINSAMP}(t+1, \s_{\phi_{t+1}})$.

Second, one can sample node $v_i$ and compute $s_{v_i}$ as:
\begin{align}
s_{v_i} &= \frac{c_{v_i} + 1 - \delta_{\min}}{r_{v_i}}   
\label{eq:scale1}
\end{align}
The cost for this choice is $c_1 = 1 + \texttt{MINSAMP}(t+1, \s_{\phi_{t+1}})$.
The algorithm then returns the smaller value between $c_0$ and $c_1$.

If $c_{v_i} - r_{v_i} < \delta_{\min}$, then one has no choice but to sample node $v_i$ so that left-end of disc $v_i$ is at least $\delta_{\min}$. 
Scale factor $s_{v_i}$ must be computed using \eqref{eq:scale1}, and the algorithm returns $c_1$. 
The pseudo-code of the algorithm is shown in Algorithm\;\ref{algo:DP}.

\begin{algorithm}
\caption{compute minimum sample count given $\delta_{\min}$}
\begin{algorithmic}[1]
\Procedure{\texttt{MINSAMP}}{$t, \s_{\phi_t}$}
\State $r_{v_t} \gets \sum_{j \neq i} \frac{L_{i,j}}{s_j}$ 
\If{$c_{v_t} - r_{v_t} > \delta_{\min}$}
\State $s_{v_t} \gets \frac{c_{v_t} - \delta_{\min}}{r_{v_t}}$ 
\Comment{\textbf{Choice 0}: don't sample $v_t$}
\State $\s_{\phi_{t+1}} \subseteq \s_{\phi_t} \cup \{s_{v_t}\}$
\Comment{Define scale factors of $\phi_{t+1}$}
\If{t < N}
\State $c_0 \gets \texttt{MINSAMP}(t+1,s_{\phi_{t+1}})$
\Else
\State $c_0 \gets 0$
\EndIf
\Else
\State $c_0 \gets \infty$
\EndIf
\State $s_{v_t} \gets \frac{c_{v_t} +1 - \delta_{\min}}{r_{v_t}}$
\Comment{\textbf{Choice 1}: sample $v_t$}
\State $\s_{\phi_{t+1}} \subseteq \s_{\phi_t} \cup \{s_{v_t}\}$
\Comment{Define scale factors of $\phi_{t+1}$}
\If{t < N}
\State $c_1 \gets 1+ \mathtt{MINSAMP}(t+1,s_{\phi_{t+1}})$
\Else
\State $c_1 \gets 1$
\EndIf
\State \textbf{return} $\min (c_0, c_1)$
\Comment{Return smaller of two choices}
\EndProcedure
\end{algorithmic}
\label{algo:DP}
\end{algorithm}

Algorithm\;\ref{algo:DP} is a recursive algorithm that runs in exponential time.
To create overlapping sub-problems and enable DP, as done in \cite{cheung07transcsvt} we first \textit{quantize} each scale factor $s_i$ in $\s_{\phi_{t}}$ to $K$ discrete values givren step size $\zeta$:
\begin{align}
x_i = \left\lfloor 
\frac{s_i}{\zeta} \right\rfloor
\end{align}
Each time a recursive call $\texttt{MINSAMP}(t,\s_{\phi_t})$ is called, the computed solution is stored in entry $[t][z_i] \ldots$, $i \in \phi_t$, of a DP table, so that a subsequent call to $\texttt{MINSAMP}(t,\s_{\phi_t})$ can simply retrieve the computed value from the DP table.
The complexity of Algorithm\;\ref{algo:DP} is then the size of the DP table times the time required to compute each entry in the table, which is $O(N K^D)$, where $D$ is the maximum size of $\phi_t, \forall t$.


\subsection{Disc Threshold Search}
\label{subsec:singular}

We discuss the problem of finding a disc threshold $\delta_{\min}$ such that the optimal solution $(\{s_i^*\}, \{e_i^*\})$ to (\ref{eq:discAlign2}) satisfies $\sum_{i=1}^N e_i^* = \bar{H}$, denoted as $\bar{\delta}_{\min}$.
First, one can show that the sample count $H(\delta_{\min}) = \sum_{i=1}^N e_i^*$ of the optimal solution to (\ref{eq:discAlign2}) is a non-decreasing function with respect to threshold $\delta_{\min}$.
(See Appendix\;\ref{subsec:append2} for a short proof.)
Given also that $\delta_{\min} \geq 0$, one simple strategy to find $\bar{\delta}_{\min}$ is to perform \textit{binary search} on the non-negative number line $[0, \infty)$.
This is indeed the approach we pursue when $H(\delta_{\min})$ is far from $\bar{H}$.

When $H(\delta_{\min})$ is close to $\bar{H}$, small adjustments to $\delta_{\min}$ may induce no changes in $H(\delta_{\min})$, and the number of search iterations until $\bar{\delta}_{\min}$ is discovered is not bounded \textit{a priori}. 
We thus pursue a strategy known as \textit{singular threshold}. 
The notion of singular threshold has been studied extensively in the context of bit allocation problems for signal compression
\cite{shoham88,cheung00,deabreu18}.
In its simplest form, a finite budget of $\bar{H}$ discrete source coding bits are divided among a set of $K$ quantizers as $h_1, \ldots, h_K$, so that the sum of distortions $d_k(h_k)$'s among the $K$ quantizers is minimized, \textit{i.e.},
\begin{align}
\min_{\{h_k\}} \sum_{k=1}^K d_k(h_k)
\;\;\; \mbox{s.t.} \;\;
\sum_{k=1}^K h_k \leq \bar{H}
\label{eq:primal}
\end{align}
The constrained resource allocation problem is converted to an unconstrained one using Lagrangian relaxation with Lagrange multiplier $\lambda$, \textit{i.e.},
\begin{align}
\min_{\{h_k\}} \sum_{k=1}^K d_k(h_k) + \lambda h_k
\label{eq:dual}
\end{align}
For fixed $\lambda$, the unconstrained problem can be solved efficiently.
The problem is how to find multiplier $\lambda$ such that the optimal solution to the Lagrangian dual $\{h_k^*\}$ has rate $H = \sum_{k=1}^K h_k^*$ equals to the budget $\bar{H}$ (if possible), in which case the Lagrangian solution $\{h_k^*\}$ to (\ref{eq:dual}) is also optimal to the constrained problem (\ref{eq:primal}).

\vspace{0.0in}
\begin{figure}[t]%[h]
\begin{center}
\includegraphics[width=2.2in]{figures/singularSearch.png}
\vspace{-0.1in}
\caption{Example Search for $\delta_{\min}$ using Singular Thresholds}
\label{fig:singularSearch}
\end{center}
\end{figure}

Towards this goal of finding an appropriate $\lambda$, the authors in (\cite{shoham88}) defined a notion of \textit{singular threshold}, which is a particular value of $\lambda$ at which there exist \textit{multiple} optimal solutions to (\ref{eq:dual})  



==> tableAbb.tex <==
\begin{table}
\caption{Details for Abbreviations used in Performance  Figures}
\label{analysis}
\begin{center}
\begin{tabular}{c|c|c}
% ????????????????????????????????????????????????????
% \toprule %???????
 \hline
\hline
  \textbf{}&{Sampling}&{Reconstruction}\\\hline
random-G&random& GLR \eqref{eq:obj0} \\\hline
PG-LS&PG \cite{PG}& Least Squares in \cite{PG}\\\hline
PG-G&PG \cite{PG}& GLR \eqref{eq:obj0}\\\hline
%Ao-LS2&A-optimal \cite{PG}& Least Squares in \eqref{AoptimalMC}\\\hline
%AoL-LS2&A-optimal \cite{PG}; Local search pool& Least Squares in \eqref{AoptimalMC}\\\hline
AoL-G&A-optimal \cite{PG}; Local search pool& GLR \eqref{eq:obj0}\\\hline
GCS-G&GCS& GLR \eqref{eq:obj0}\\\hline
IGCS-G&IGCS& GLR \eqref{eq:obj0}\\\hline
 \end{tabular}
 \end{center}
\end{table}

==> tableBLSM.tex <==
\begin{table*}
\caption{Graph Sampling for Active Matrix Completion}
\label{analysis}
\begin{center}
\begin{tabular}{c|c|c|c|c|c}
% ????????????????????????????????????????????????????
% \toprule %???????
 \hline
\hline
  \textbf{}&{Input}&{Unstructured?}&Candidate number& Evaluation on per Candidate&Assumption\\\hline
PG \cite{PG}&$\U$;$\V$&No&$\cO(m+n)$&$\cO()$&Bandlimitedness\\\hline
SP \cite{anis16} &$\L_p$& Yes &$\cO(1)$&$\cO(kmnR(k))$&Bandlimitedness\\\hline
{E-optimal} &$\U$;$\V$&Yes&$\cO(mn)$&$\cO(k^3_1k^3_2)$&Bandlimitedness\\\hline
A-optimal&$\U$;$\V$&Yes&$\cO(mn)$&$\cO(k^3_1k^3_2)$&Bandlimitedness\\\hline
Proposed GCS&$\L_r$;$\L_c$&Yes&$\cO(1)$&$\cO(Rmn)$&Smoothness\\\hline
Proposed IGCS&$\L_r$;$\L_c$&Yes&$\cO(1)$&$\cO({R_0}\max\{m,n\})$&Smoothness\\\hline
 \end{tabular}
 \end{center}
\end{table*}
